Learning to Follow Instructions in Text-Based Games

Text-based games present a unique class of sequential decision making problem in which agents interact with a partially observable, simulated environment via actions and observations conveyed through natural language. Such observations typically include instructions that, in a reinforcement learning (RL) setting, can directly or indirectly guide a player towards completing reward-worthy tasks. In this work, we study the ability of RL agents to follow such instructions. We conduct experiments that show that the performance of state-of-the-art text-based game agents is largely unaffected by the presence or absence of such instructions, and that these agents are typically unable to execute tasks to completion. To further study and address the task of instruction following, we equip RL agents with an internal structured representation of natural language instructions in the form of Linear Temporal Logic (LTL), a formal language that is increasingly used for temporally extended reward specification in RL. Our framework both supports and highlights the benefit of understanding the temporal semantics of instructions and in measuring progress towards achievement of such a temporally extended behaviour. Experiments with 500+ games in TextWorld demonstrate the superior performance of our approach.

==> coverpage.tex <==
\section*{{\Large Team Communication}}

\subsection*{Comment formats}

\maybe{This is a text that's a maybe} - \revisit{This is text to revisit} - \added{This is an added text}  - \remove{This should be removed} - \commenttk{This is an inline comment by TK. (Analogous macros for SM, SS, MT, AL, PV)}\\
\maybecomment{This is a text that's a maybe with a comment}{this is a comment or just a general thought - adding 'comment' after the above commands will achieve the same thing for each type of command}\\
% \revisit{This is text to revisit} -- ``revisit'' is intended for things we need to check later. It can be used, for example to highlight things we're not sure we really ended up doing (so may wish to remove or de-emphasize).\\
% \comment{This is the text to comment}{this is a comment}\\
% \added{This is an added text}\\
% \addedcomment{This is an added text with a comment}{this is a comment}\\
% \remove{This should be removed}\\
% \removecomment{This should be removed with a comment}{this is a comment}\\
% \commenttk{This is an inline comment by TK. (Analogous macros for SM, SS, MT, AL, PV)}

% \subsection*{Communications}
% \begin{itemize}
%     \item -
% \end{itemize}

% \subsection*{To Do's}
% \begin{itemize}
%     \item -
% \end{itemize}
\section*{Page Layouts + Polishing}
8 page total, not including (1) references (2) broader impact (3) appendix

\begin{itemize}
    \item $2$ pages: Abstract + Introduction
    \item $1$ pages: background : \revisit{this section is currently 2 pages}
    \item $\sim 2/3$ page: expose
    \item $1.5$ pages: method \revisit{this section is currently 2.5 pages}
    \item $2$ pages: experiments \revisit{this section is currently 3.5 pages}
    \item $0.5 page$: related works
    \item $\sim 1/3$ page: conclusion
\end{itemize}
\subsection{Additional notes}
\begin{itemize}
    \item who's doing what section
    \item pitch
    \item introduction: follow structure of abstract
    \item limitations + broader impact
    \begin{itemize}
        \item -
    \end{itemize}
    \item section 5 \commenttk{This might be section 4 now -- I removed the number from the section on the current page.}
    \begin{itemize}
        \item LTL is an internal structured representation that allows us to study instruction following, exploit the temporal semantics
        \item we translate instructions to LTL, augment the architecture
        \item 
    \end{itemize}
\end{itemize}

\newpage

\subsection*{Framing the Paper}
\commentmt{feel free to amend. Wanted to put something here so we are all consistent on the "vision"}
\begin{itemize}
    \item {\color{blue} introduction} We perform a scientific study - and in turn, show how using formalized instructions with "progression" (some means of monitoring) can achieve sota performance.
    \begin{itemize}
        \item Through this study, we identify how current sota (GATA) ignores instructions (Fig 2)
        \item GATA doesn't compelte tasks well (success rate vs. points)
        \item It has no goal understanding, tracking, etc, and it's left to act erroneously until/if the goal is achieved
        \item Ideally, an agent should read the natural language and understand/follow the instructions, but even like a human, you \textit{do} need some mechanism for remembering these instructions and monitoring your progress
        \item (aside: In an ideal world, a language model might be able to to do this end-to-end)
        \item However, there are a lot of potentialy benefits to a formal internal form (progression, no memory?, interpretability? simplicity - we achieve this without a huge transformer?)
    \end{itemize}
    \item Instructions are not necessarily reward-bound (i.e. examining the cookbook)
    \item We propose using LTL to formalize these instructions and monitor our progress in achieving them
    \item We take the GATA model and augment it to additionally condition on these instructions (this should be layed out prior to rest of paper)
    \item {\color{blue} background} We then present some background material
    \item {\color{blue} expose} We then present the expose \commentmt{I have the expose \textit{after} background because of some details like the game description and stuff that I wanted to cover before the expose. Perhaps this is not best ordering, welcome to suggestions.}
    \item {\color{blue} LTL} We then present LTL and progression
    \item {\color{blue} method} We then present our method
    \begin{enumerate}
        \item how LTL formalizes instructions
        \begin{itemize}
            \item How we can 'automatically' generate them from the observations
            \item How we format them
        \end{itemize}
        \item How LTL reward works, and how we can terminate episodes \textit{if} an LTL instruction is violated
        \item We present the \textit{new} model, i.e. the augmentation over the GATA model.
    \end{enumerate}
    \item {\color{blue} experiments}
    \begin{itemize}
        \item Covers setup and hyper-parameters
        \item Cover level performance
        \item Cover ablations
        \item Try and think of arguments against work and identify them before reviewer does
    \end{itemize}
    \item {\color{blue} related works}
    \item {\color{blue} conclusion}

\end{itemize}
\setcounter{page}{0}

==> coverpageCRC.tex <==
\section*{{\Large CRC Things to Remember}}

\begin{itemize}
    \item Revisit "generalization" section in experiments that we commented out
    \item See if we can get rid of the "TBG" abbreviation
    \item Consider further linkages to other work on instruction following, and our reflections on the merit of abstraction and evaluation of NLP propositions or sentences.
    \item Future work discussion in conclusion
\end{itemize}

\setcounter{page}{0}

==> sections/broader-impact.tex <==
\section{Broader Impact}
\cite{adhikari2020learning} and \cite{liu2022learning} identify important social impacts of this area of work, and we would like to build on their discussion. We identify that text-based are a good proxy for studying human-machine interaction through language. Human-machine interaction and relevant systems have many potential ethical, social, and safety concerns:
\begin{itemize}
    \item Providing inaccurate policies or information in critical systems can have devastating consequences. For example, in health care, improper treatment can be fatal, or in travel planning, poor interaction can lose a client money.
    \item Providing efficient, well structured policies in fields such as customer service or online shopping can greatly improve the user experience.
    \item Partial completion of tasks can also have serious safety concerns. Imagine an agent tasked with helping a person cross a street, and only taking them half way. OR issues with partial completion on user experience.
\end{itemize}

\cite{adhikari2020learning} correctly identified that work in this area should (a) improve in the ability to make better decisions, (b) constrain decisions for safety or other, and (c) improve interpretability. We highlight how RL agents equipped with LTL instructions can improve in these areas. On interpretability specifically, we identify how monitoring the progression of instructions provides a mechanism for understanding where and when an agent might be making incorrect decisions, and provides the opportunity to revise instructions or attempt to fix the problem by other means. Further, we would like to that works towards building better language agents should also emphasize the completeness of instructions. To that end, we have proposed using game success rate as a baseline metric for future work and demonstrated how \agentname\ is very successful in the games it plays, and consistently outperforms state-of-the-art.

\commenttk{This section seems to avoid directly addressing ``potential negative societal impacts of your work''. I think we should be able to come up with something a bit more specific to our work. Maybe something about how an agent which follows instructions too literally might not achieve the behavior that is actually desired in some cases. Maybe something about social norms (\url{https://arxiv.org/abs/2205.01975}), which we don't try to address?}

==> sections/old-butrecent-introduction.tex <==
\section{Original Introduction}
\label{sec:introduction}


% \begin{itemize}
%     \item core issues/gap
%     \begin{itemize}
%         \item agents can't follow instructions
%         \item belief states are researched and needed but don't solve the fundamental problem of semantic disconnect
%         \item there is semantic disconnect between observations/state and actions, all represented in text
%     \end{itemize}
%     \item claim/our work
%     \begin{itemize}
%         \item to finish the puzzle, we propose using LTL to help agents follow instructions
%         \item LTL provides a platform to understand text and a mechanism for semantic connection through progression (changes in observations/choices in actions tied to progression in LTL formula that represent goals)
%     \end{itemize}
%     \item support (experimental)
%     \begin{itemize}
%         \item higher performance on lower levels in 20-game, and much higher performanec on lower levels in 100-game
%         \item gata fails in simple complexity increases
%         \item gata performs the same even when instructions are stripped from observations (it's not paying attention to them)
%         \item even just feeding the goal as text is not enough, the mechanism of LTL are needed.
%         \item performance even without rewrad for LTL satisfaction is almost unaltered, showing that its more about the augmented state than the reward scheme
%     \end{itemize}
%     \item Method
%     \begin{itemize}
%         \item we employ a double DQN model
%         \item text is encoded using a basic transformer
%         \item LTL is represented as text to the agent and processed internally in its raw logical form
%         \item we concatenated observations + ltl + states rather than use any complex feature aggregation method
%         \item 
%     \end{itemize}
% \end{itemize}

% Sheila: 
% - instructions play two different roles: (1) both instructions as we might classically interpret them and (2) more informally as advice.
% - how to separate navigational failures from instruction-following failures
% - take-aways: (1) need to pay attention to instructions (and have a digestible form of instructions that the RL learner can predict from), (2) need to measure progress.
%
% Pashootan:
% - future work (conclusions): use KG / observations to attend to LTL, might remove need for explicit progression (is this good or bad?)
% - measuring useful / non-useful actions (especially in higher levels)
%
% Mat:
% - future work: (1) inability to abstract over training examples and (2) navigate hurts test time performance in higher levels.  (3) lack of systematic exploration to information gather... how to explore optimally in these PO domains?

Getting agents to understand text is a long-standing problem in artificial intelligence, and recently the problem of getting reinforcement learning (RL) agents to play text-based games has been a popular challenge \citep{cote2018textworld, adhikari2020learning, liu2022learning}. Text-based games present a unique, partially observed interactive natural language simulation involving a sequential decision making problem where agents are required to interpret text-based observations and act using text-based actions. Successful play requires good language understanding, efficient navigation, good memory, and an ability to follow instructions embedded within the text \citep{cote2018textworld}. Text-based Games can be viewed as a proxy-environment for task-oriented dialogue \citep{budzianowski2018multiwoz}, where RL agents must interpret a user's text-based requests and make decisions on how to respond. 

The fundamental challenge of text-based games is to teach RL agents to understand natural language. Rooted in that challenge is the need for agents to understand, remember, and follow \emph{instructions} that are present within the text-based observations of a game. Instructions may or may not be bound to an \revisit{intrinsic} reward, but can directly or indirectly guide an agent towards completing tasks and its goal. In this work, we study the ability of RL agent to remember and follow these instructions. 

Recent works, in particular the model-based state-of-the-art agent GATA \cite{adhikari2020learning}, have focused on developing long-term memory to solve these games. Despite GATA's improvement over baselines, the agent generally ignores instructions and is unaffected when instructions are stripped from  game play. We show this experimentally in \autoref{fig:stripped}. Intuitively, without knowing the goal or following instructions to achieve the goal, agents couldn't reasonably succeed in solving these games. This becomes very clear examining GATA's performance on Level 2 in \autoref{fig:stripped}, where the success rate of games is around half of the normalized game points it actually achieves. \commentmt{writers block for how to write this part. also add more on the new measure we have here.}



We wish to bring attention to the importance of following instructions in text-based games. \remove{and demonstrate how to teach text-based agents to follow instructions using Linear Temporal Logic (LTL)} 
%\commenttk{I'm not sure readers will understand what LTL is being used for from that sentence (it has the same form as, e.g., ``teach text-based agents to follow instructions using curriculum learning''.} \commentmt{agreed. see ->} 
\added{We demonstrate how to teach text-based agents to follow instructions by equipping RL agents with an internal structured representation in the form of Linear Temporal Logic (LTL) of the instructions found within the natural language.}. LTL is a formal modal logic with time-based modalities and binary predicates that dictate the events of the world (e.g. have-apple). LTL is able to expressively represent goals (or sequences of goals) and can -- through a mechanism called \textit{LTL progression} -- update goals that are yet to be satisfied while preserving the semantics of the original goal(s).
% \rephrase{LTL is an expressive formal language that combines temporal modalities such as eventually, until, and always with binary predicates that establish the truth or falsity of an event or property (e.g., have-coffee), composed via logical connectives to support specification of goal sequences, partial-order tasks, safety constraints, and much more. Our learning algorithm exploits a semantics-preserving rewriting operation, called LTL progression, that allows the agent to identify aspects of the original instructions that remain to be addressed in the context of an evolving experience.} 
%\remove{permits agents to learn the causal effects of their text-based actions through progression, which}
\revisit{We augment the GATA model using LTL to} allow it to condition on this structured representation over time and hypothesize that through progression, LTL  enables agents to \revisit{learn to follow instructions}. Our contributions are as follows:
\begin{itemize}
    % \item We in introduce a framework for teaching text-based RL agents how to follow instructions using LTL, built of \comment{LTL2Action}{Pop to a higher-level discussion of needing a symbolic representation of instructions and progression to inform the decision-making.} \cite{vaezipoor2021ltl2action}.
    \item We present our findings that show how current agents fail to follow instructions, leading to uninformed decision making in text-based games.
    \item We demonstrate the benefits of a formal representation of instructions (using LTL) for more informed decision-making in text-based games. We show how this approach greatly improves performance over state-of-the-art without increasing model complexity. \commentmt{Do we want to argue the "model complexity" as another benefit? If not remove this sentence maybe. }
    % \commenttk{Demonstrating that a formal representation of instructions improves performance doesn't mean that such a representation was \emph{needed}.\commentmt{Good point, changed to benefits}}
    \item We further show how the use of LTL progression is \added{a} critical mechanism that enables agents to realize their goals.
    % \item \added{We introduce a novel episodic exploration reward based on the set of environment objects that are relevant to the agent's goal?}
    % \item We demonstrate how this approach greatly improves performance over state-of-the-art. \commenttk{Maybe this should be part of the second point? Are the benefits referred to there different from greatly improved performance?}
\end{itemize}

==> sections/old_background.tex <==
\section{Background}
\label{sec:background}

\subsection{Text-Based Games: TextWorld}
\label{sec:text_based_games}
Text-based games (TBG) are partially observed multi-turn games built using natural language. In this work, we use TextWorld as our text-based game engine \footnote{Henceforth, TextWorld and Text-Based Games may be used interchangeably}. TBGs are well formulated under the RL formalism, and can be viewed as the discrete-time POMDP $<S, T, A, O, \Omega, R, \gamma>$ \citep{cote2018textworld} where $S$ is the environment's state space, $A$ is the action space, $T(s_{t+1} | s_t, a_t)$ where $s_{t+1}, s_t \in S$ and $a_t \in A$ is the conditional transition probability between states $s_{t+1}$ and $s_t$ given action $a_t$, $O$ is the set of (partial) observations that the agent receives, $\Omega(o_t | s_t, a_{t-1})$ is the set of conditional observation probabilities, $r_t = R(s, a) : S \times A \rightarrow \mathbb{R}$ is the reward function for state action pair $(s, a)$, and $\gamma \in [0, 1]$ is the discount factor. The goal for an RL agent is to learn some optimal policy $\pi^*(a | s)$ that maximizes the expected discounted return. Text-based games are played one of three ways: (1) choice-based games where an agent selects from a choice of actions at each step in an episode: (2) hypertext-based games where an agents clicks on one of several links from the current text observations: (3) parser-based games where agents must type text commands chosen from a predefined vocabulary to compose commands \citep{cote2018textworld}. In this work, we focus on choice-based games similar to previous works \citep{adhikari2020learning, liu2022learning, narasimhan2015language}. In this case, our action space $A$ is a list of possible commands and at each time-step $t$ in the game, the agent must select action $a_t \in C_t$ from the current subset of permissible actions $C_t \subset A$. \commentmt{should we ref. the data-flow figure (fig 2) here?}.

\subsubsection{Environment Setting}
\commentmt{@Toryn, the ICLR work cited the original textworld paper, GATA cited no one and said "similar" like me, the problem is the original TW paper only talks about coin collection game, and the cooking game is part of their "benchmarks" but it's not mentioend in the original paper. It can be found in their python docs though}
We focus on the popular \textit{Cooking Domain} (\comment{similar to}{TK: Is there somewhere we can cite for the game itself, instead of just something it's similar to?} the games used in Microsoft's \textit{First TextWorld Problems: A Language and Reinforcement Learning Challenge} (FTWP)), in which agents must gather and prepare various cooking ingredients described by an in-game recipe that is to be found. Game points (rewards) are earned by some combination of (1) collecting the proper ingredients, (2) preparing them (preparation can involve some cutting action and/or some cooking action), (3) preparing the meal once all of the ingredients have been prepared, and (4) eating the meal. \added{The in-game observations contain instructions that will describe how to succeed in each game instance, but importantly not all instructions lead to reward. Critically, an agent in this game is first instructed to examine a cookbook which elicits a recipe to be followed. The act of examining the cookbook returns no reward, but following this recipe will return reward. See \autoref{sec:app_tw} for more details.} Success is determined by whether the recipe is fully completed. Preparing ingredients can also involve collecting certain tools (e.g., a knife). The game may also involve navigation, where an agent may need to navigate to the kitchen or navigate to find certain ingredients.


\subsection{Linear Temporal Logic (LTL)}
\label{sec:ltl}
Linear Temporal Logic (LTL) is a temporal first-order logic with time-based modalities. It is composed of (a) propositional variables (e.g. player-has-carrot), (b) logical operators (e.g. $\neg$), and (c) two temporal operators: $\ltlnext$ ($\ltlnextTXT$) and $\textltluntil$ ($\ltluntilTXT$). Formally, we define the syntax of LTL per \cite{DBLP:books/daglib/0020348} as
\begin{equation*}
    \varphi \Coloneqq p \;|\; \neg \varphi \;|\; \varphi \wedge \psi \;|\; \ltlnext \varphi \;|\; \varphi \ltluntil \psi
\end{equation*}

where $p \in \mathcal{P}$ for some finite set of propositional symbols $\mathcal{P}$.
Satisfaction or realization of an LTL formula is determined by the sequence of truth assignments $\sigma=\langle \sigma_0, \sigma_1, \sigma_2, \ldots \rangle$ for $\mathcal{P}$, where $p \in \sigma_i$ iff proposition $p \in \mathcal{P}$ holds at time step $i$. Formally, denoted as $\tuple{\sigma,i}\models\varphi$, $\sigma$ \emph{satisfies} $\varphi$ at time $i \geq 0$, as:
\begin{itemize}
    \item $\tuple{\sigma,i}\models p$ iff $p\in \sigma_i$, where $p \in \mathcal{P}$
    \item $\tuple{\sigma,i}\models \neg \varphi$ iff $\tuple{\sigma,i}\not\models\varphi$
    \item $\tuple{\sigma,i}\models (\varphi\wedge\psi)$ iff $\tuple{\sigma,i}\models\varphi$ and $\tuple{\sigma,i}\models\psi$
    \item $\tuple{\sigma,i}\models\ltlnext\varphi$ iff $\tuple{\sigma,i+1}\models\varphi$
    \item $\tuple{\sigma,i}\models\varphi\ltluntil\psi$ iff there exists $j$ such that $i\le j$ %\le n$ % removed per Sheila's comment
    and\\%\verb!     ! %\verb command causes an error inside a colored region
    $\tuple{\sigma,j}\models\psi$, and $\tuple{\sigma,k}\models\varphi$ for all $k \in [i,j)$
\end{itemize}

A sequence $\sigma$ is then said to \emph{satisfy} $\varphi$ iff $\tuple{\sigma,0}\models\varphi$.

Any LTL formula can be defined in terms of $p \in \mathcal{P}$, $\wedge$ (\emph{and}), $\neg$ (\emph{negation}), $\ltlnext$ ($\ltlnextTXT$), and $\textltluntil$ ($\ltluntilTXT$). From these operators, we can also define the Boolean operators $\vee$ (\emph{or}) and $\rightarrow$ (\emph{implication}), and the temporal operators $\ltlalways$ ($\ltlalwaysTXT$) and $\ltleventually$ ($\ltleventuallyTXT$), where $\tuple{\sigma,0}\models\ltlalways \varphi$ if $\varphi$ always holds in $\sigma$, and $\tuple{\sigma,0}\models\ltleventually \varphi$ if $\varphi$ holds at some point in $\varphi$.



% \rephrase{Linear Temporal Logic (LTL) extends propositional logic with two temporal operators: $\ltlnext$ (\emph{next}) and $\textltluntil$ (\emph{until}). Given a finite set of propositional symbols $\mathcal{P}$, the syntax of an LTL formula is defined as follows \cite{DBLP:books/daglib/0020348}:
% \begin{equation*}
%     \varphi \Coloneqq p \;|\; \neg \varphi \;|\; \varphi \wedge \psi \;|\; \ltlnext \varphi \;|\; \varphi \ltluntil \psi \text{ ~~~~where $p \in \mathcal{P}$}
% \end{equation*}
% In contrast to propositional logic, LTL formulas are evaluated over sequences of observations (i.e., \emph{truth assignments} to the propositional symbols in $\mathcal{P}$). Intuitively, the formula $\ltlnext \varphi$ (\textit{next} $\varphi$) holds if $\varphi$ holds at the next time step and $\varphi \ltluntil \psi$ ($\varphi$ \textit{until} $\psi$) holds if $\varphi$ holds until $\psi$ holds. 

% %\begin{definition}[LTL semantic]
% %\end{definition}
% Formally, the truth value of an LTL formula is determined relative to an infinite sequence of truth assignments $\sigma=\langle \sigma_0, \sigma_1, \sigma_2, \ldots \rangle$ for $\mathcal{P}$, where $p \in \sigma_i$ iff proposition $p \in \mathcal{P}$ holds at time step $i$. Then, $\sigma$ \emph{satisfies} $\varphi$ at time $i \geq 0$, denoted by $\tuple{\sigma,i}\models\varphi$, as follows:
% \begin{itemize}
%     \item $\tuple{\sigma,i}\models p$ iff $p\in \sigma_i$, where $p \in \mathcal{P}$
%     \item $\tuple{\sigma,i}\models \neg \varphi$ iff $\tuple{\sigma,i}\not\models\varphi$
%     \item $\tuple{\sigma,i}\models (\varphi\wedge\psi)$ iff $\tuple{\sigma,i}\models\varphi$ and $\tuple{\sigma,i}\models\psi$
%     \item $\tuple{\sigma,i}\models\ltlnext\varphi$ iff $\tuple{\sigma,i+1}\models\varphi$
%     \item $\tuple{\sigma,i}\models\varphi\ltluntil\psi$ iff there exists $j$ such that $i\le j$ %\le n$ % removed per Sheila's comment
%     and\\%\verb!     ! %\verb command causes an error instead a colored region
%     $\tuple{\sigma,j}\models\psi$, and $\tuple{\sigma,k}\models\varphi$ for all $k \in [i,j)$
% \end{itemize}
% A sequence $\sigma$ is then said to \emph{satisfy} $\varphi$ iff $\tuple{\sigma,0}\models\varphi$.

% In order to instruct RL agents using language, the first step is to agree upon a common 
% %SM it's not always a "common" vocab, we have a translator -- the labelling function.
% vocabulary between us and the agent. In this work, we use a finite set of propositional symbols $\mathcal{P}$ as the vocabulary, representing high-level events or properties (henceforth ``events'') whose occurrences in the environment can be detected by the agent. For instance, in a smart home environment, $\mathcal{P}$ could include events such as opening the living room window, activating the fan, turning on/off the stove, or entering the living room. Then, we use LTL to compose temporally-extended occurrences of these events into instructions. For example, two possible instructions that can be expressed in LTL (but described here in plain English) are (1) ``Open the living room window and activate the fan in any order, then turn on the stove" and (2) ``Open the living room window but don't enter the living room until the stove is turned off". }
\subsection{LTL Progression}
\label{sec:prog}
In addition to expressing instructions through logic, an LTL formula can also be \textit{progressed} along a sequence of truth assignments \citep{bacchus1996rewarding, toro2018teaching}. In other words, as an agent acts in the world, resulting truth assignments can be used to update the formula to reflect what has been satisfied. This update is semantically preserving. The updated formula would now reflect the parts of the original formula that are remaining to be satisfied or whether the formula has been violated/satisfied. Formally, we define the progression operator $\mprog(\sigma_i, \varphi)$ as follows:
\begin{definition}
For LTL formula $\varphi$, truth assignment $\sigma_i$ over $\mathcal{P}$, and $p \in \mathcal{P}$, $\mprog(\sigma_i, \varphi)$ is defined as
\begin{align*}
    &\mprog(\sigma_i, \varphi) = \true~\text{if}~p \in \sigma_i\\
    &\mprog(\sigma_i, \varphi) = \false~\text{if}~p \notin \sigma_i\\
    &\mprog(\sigma_i, \neg\varphi) = \neg\mprog(\sigma_i, \varphi)\\
    &\mprog(\sigma_i, \varphi_1 \wedge \varphi_2) = \mprog(\sigma_1, \varphi_1) \wedge \mprog(\sigma_1, \varphi_2)\\
    &\mprog(\sigma_i, \ltlnextTXT\varphi) = \varphi\\
    &\mprog(\sigma_i, \varphi_1\ltluntilTXT\varphi_2) = \mprog(\sigma_1, \varphi_2) \vee (\mprog(\sigma_1, \varphi_1) \wedge \varphi_1 \ltluntilTXT \varphi_2)
\end{align*}
\end{definition}

In the context of TextWorld, the progression operator can be applied at every step in the episode to update the LTL instruction given to the agent. For example, the LTL instruction $\varphi : \ltleventuallyTXT \ltlpredicate{player-has-carrot} \wedge \ltleventuallyTXT \ltlpredicate{player-has-apple}$ would be progressed to $\ltleventuallyTXT \ltlpredicate{player-has-apple}$ once the agent grabs the carrot during an episode. In other words, when the agent reaches a state where $\ltlpredicate{player-has-carrot}$ is true, the LTL instruction is progressed to reflect that the agent must now still grab the apple at some point in the future. % Note that if at some later point the agent drops the carrot, the LTL formula will not be updated and regress to its previous form. This is because in the sequence\commentmt{confirm this and be sure of whether we want to inclde this}

In order for progression to occur, it becomes necessary to have some \textit{event detector} that can detect these truth assignments as the agent acts during an episode. We discuss how event detection occurs in the subsequent sections.

==> sections/old_following-instructions.tex <==
\section{Following Instructions}
% \subsection{Ignoring Instructions}

\commentsm{Moving here for now.  Used to be Section 2.2. "Ignoring Instructions"}
%\commentmt{move section: I originally put here because of some details in here that I felt necessary to cover (i.e. POMDPs, textworld environment, etc. Given that, I'm not sure the best place to put this section}
% \commentmt{yes ICLR is a model-based method. I have found a couple non-published works that report slightly better results here and there, but nothing with usable code or published. Further, some odd reporting (like different games, etc.) which makes me question it. Further, the ICLR work uses GATA as their baseline as well, which tells me they also didn't find anything else (or chose to exclude it). There's some other works, not applied to textworld but other TBG, but not stellar results necessarily above GATA's, and aren't compatible with TextWorld (the env doesn't provide certain info they need).}
% \comment{To date}{TK: Will that still be true at submission time, which is after ICLR?} 
To date, the state-of-the-art (SOTA) model-free RL agent for TextWorld is the Graph Aided Transformer Agent (GATA) \citep{adhikari2020learning}. GATA uses a transformer variant of the popular LSTM-DQN \cite{narasimhan2015language} combined with a dynamic belief graph that is inferred and updated during planning. The aim is to use the dynamic belief graph to improve action selection by modelling the underlying game dynamics \citep{adhikari2020learning}. Formally, given the POMDP $<S, T, A, O, \Omega, R, \gamma>$, GATA attempts to learn some optimal policy $\pi^*(a | s, g)$ where $g$ is the belief graph of the agent.

GATA is among the popular trend \citep{ammanabrolu2020graph, zelinka2019building, ammanabrolu2018playing} of using a form of memory to augment an agent's state space. This is indeed an important problem and critical to solving these partially observed TBGs \citep{cote2018textworld}, however we argue that this is not the full picture. Even with the inclusion of memory, GATA fails to follow even the simplest of instructions within the environment which leads to poor performance. 
%Thi. Memory is critical because it allows the agent to recall its past behaviour to hopefully more informed decisions in the future, and in a partially observed environment like TextWorld, this is vital. Further, focusing on GATA, it has the ability capture goal-related relations like `needs` (e.g. apple-needs-cut). However despite GATA capturing such relations, and despite the observations containing instructions that, if followed, will lead the agent towards success, current agents ignore these instructions and fail to properly follow instructions. 

Despite works like GATA that even capture goal relations (e.g. apple-needs-cut), agents trained to condition on observations and belief state alone fail to handle even slight increases in game complexity and completely ignore in-game instructions that \textit{should} lead the agent to success. To highlight this, in \autoref{tab:recipe} we tabulate the frequency and at which average step the GATA agent opens the cookbook in the Cookbook domain to read the recipe for various game levels. Note how it almost never does examine the cookbook, and if it does, it's later in the episode, meaning the agent was acting \comment{aimlessly}{TK: Well, maybe it was doing useful exploration?} prior to that point. In short, the GATA agent usually doesn't learn what the recipe is for the current game, meaning it has no way of knowing what the actual goal of the game is. This leads to significant performance drop-offs with even the slightest increase in game complexity. We can see this when analyzing the performance of GATA in \autoref{fig:stripped} when moving from Level $1$ to Level $2$ in the Cooking domain, where the games' complexity increases by one added task (see \autoref{tab:levels}).

% {This could be read as suggesting that you train several GATA-like agents, which I don't think is what was meant.}
We can further investigate how GATA agents fail to follow instructions by training these agents using modified game observations that have their instructions stripped. This has two effects: (1) the agent no longer receives text-based instructions about what the goal is or what it should do; and (2) GATA's belief state will no longer capture goal relations like `needs'. We visualize the results of this experiment in \autoref{fig:stripped}. Our results demonstrate how GATA's performance remains effectively constant. This highlights how GATA (a) ignores text-based instructions that would lead it to success and (b) even ignores the goal-related relations in its own belief state. 
% \commenttk{Are those goal-related relations populated correctly in the rare cases when the agent does read the cookbook?} \commentmt{more or less, it captures which ingredients need cutting/cooking, but doesn't capture the fact that the meal should be consumed. }

Although the attention on developing good belief graphs is important, it is only part of the solution for solving these text-based games. We require an additional framework that can not only model instructions or goals but also permit the agent to attend to them and know when it's successfully completing them. For this we propose Linear Temporal Logic. 


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/expose/stripped_instructions_20_games_level_1_test_bars.png}
%     \includegraphics[width=0.3\textwidth]{figures/expose/stripped_instructions_100_games_level_1_test_bars.png}
%     \includegraphics[width=0.3\textwidth]{figures/expose/stripped_instructions_100_games_level_2_test_bars.png}
%     \caption{Comparison of GATA performance when instructions are stripped from environment observations. GATA-GTP represents model trained using normal observations, and GATA-GTP* is the model trained on the stripped observations. GATA-GTP* does not capture goal relations like 'needs', and despite also not having instructions, it is equally performant to GATA-GTP.}
%     \label{fig:stripped}
% \end{figure}

\begin{table}[t]
    \centering
    \caption{\commentmt{not sure how to fomat this table}The average frequency and average game step per episode at which GATA agents examine the cookbook to elicit the game's recipe on test games. Without examining the cookbook, there is no way to know what the recipe/objective of the game is. The agent would effectively need to guess right in order to succeed without knowing the recipe.}
    \begin{tabular}{c|c|c}%{||c|c|c|c||} % Per https://media.neurips.cc/Conferences/NeurIPS2022/Styles/neurips_2022.pdf, tables should not contain vertical rules

         \toprule%\hline
         \multicolumn{3}{c}{(Frequency, Game Step)}\\
         \midrule
         Level 1&Level 2&Level 3  \\
         \midrule
         $(0, \text{N/A})$&$(0.2, 9)$&$(0, \text{N/A})$\\
         \bottomrule %\hline
    \end{tabular}
    \label{tab:recipe}
\end{table}


==> sections/old_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\commentsm{Don't forget to mention both the lack of instruction following (fig 2) and also the lack of completion of tasks and our new metric. Also explain what the instructions are as differentiated from the reward.}
% \begin{itemize}
%     \item core issues/gap
%     \begin{itemize}
%         \item agents can't follow instructions
%         \item belief states are researched and needed but don't solve the fundamental problem of semantic disconnect
%         \item there is semantic disconnect between observations/state and actions, all represented in text
%     \end{itemize}
%     \item claim/our work
%     \begin{itemize}
%         \item to finish the puzzle, we propose using LTL to help agents follow instructions
%         \item LTL provides a platform to understand text and a mechanism for semantic connection through progression (changes in observations/choices in actions tied to progression in LTL formula that represent goals)
%     \end{itemize}
%     \item support (experimental)
%     \begin{itemize}
%         \item higher performance on lower levels in 20-game, and much higher performanec on lower levels in 100-game
%         \item gata fails in simple complexity increases
%         \item gata performs the same even when instructions are stripped from observations (it's not paying attention to them)
%         \item even just feeding the goal as text is not enough, the mechanism of LTL are needed.
%         \item performance even without rewrad for LTL satisfaction is almost unaltered, showing that its more about the augmented state than the reward scheme
%     \end{itemize}
%     \item Method
%     \begin{itemize}
%         \item we employ a double DQN model
%         \item text is encoded using a basic transformer
%         \item LTL is represented as text to the agent and processed internally in its raw logical form
%         \item we concatenated observations + ltl + states rather than use any complex feature aggregation method
%         \item 
%     \end{itemize}
% \end{itemize}

% Sheila: 
% - instructions play two different roles: (1) both instructions as we might classically interpret them and (2) more informally as advice.
% - how to separate navigational failures from instruction-following failures
% - take-aways: (1) need to pay attention to instructions (and have a digestible form of instructions that the RL learner can predict from), (2) need to measure progress.
%
% Pashootan:
% - future work (conclusions): use KG / observations to attend to LTL, might remove need for explicit progression (is this good or bad?)
% - measuring useful / non-useful actions (especially in higher levels)
%
% Mat:
% - future work: (1) inability to abstract over training examples and (2) navigate hurts test time performance in higher levels.  (3) lack of systematic exploration to information gather... how to explore optimally in these PO domains?

Getting agents to understand text is a long-standing problem in artificial intelligence, and recently the problem of getting reinforcement learning (RL) agents to play text-based games has been a popular challenge \citep{cote2018textworld, adhikari2020learning, liu2022learning}. Text-based games present a unique, partially observed interactive natural language simulation involving a sequential decision making problem where agents are required to interpret text-based observations and act using text-based actions. Successful play requires good language understanding, efficient navigation, good memory, and an ability to follow instructions embedded within the text \citep{cote2018textworld}. Text-based Games can be viewed as a proxy-environment for task-oriented dialogue \citep{budzianowski2018multiwoz}, where RL agents must interpret a user's text-based requests and make decisions on how to respond. 

The fundamental challenge of text-based games is to teach RL agents to understand natural language. Rooted in that challenge is the need for agents to understand, remember, and follow \emph{instructions} that are present within the text-based observations of a game. Instructions may or may not be bound to an \revisit{intrinsic} reward, but can directly or indirectly guide an agent towards completing tasks and its goal. In this work, we study the ability of RL agent to remember and follow these instructions. 

Recent works, in particular the model-based state-of-the-art agent GATA \cite{adhikari2020learning}, have focused on developing long-term memory to solve these games. Despite GATA's improvement over baselines, the agent generally ignores instructions and is unaffected when instructions are stripped from  game play. We show this experimentally in \autoref{fig:stripped}. Intuitively, without knowing the goal or following instructions to achieve the goal, agents couldn't reasonably succeed in solving these games. This becomes very clear examining GATA's performance on Level 2 in \autoref{fig:stripped}, where the success rate of games is around half of the normalized game points it actually achieves. \commentmt{writers block for how to write this part. also add more on the new measure we have here.}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/test-bar-plots/stripped_instructions_test_bars.pdf}
    \caption{Comparison of GATA performance when instructions are stripped from environment observations. GATA\textsuperscript{D} represents model trained using normal observations, and GATA\textsuperscript{D}-S is the model trained on the stripped observations. GATA\textsuperscript{D}-S does not capture goal relations like 'needs', and despite also not having instructions, it is equally performant to GATA\textsuperscript{D}.}
    \label{fig:stripped}
\end{figure}

We wish to bring attention to the importance of following instructions in text-based games. \remove{and demonstrate how to teach text-based agents to follow instructions using Linear Temporal Logic (LTL)} \commenttk{I'm not sure readers will understand what LTL is being used for from that sentence (it has the same form as, e.g., ``teach text-based agents to follow instructions using curriculum learning''.} \commentmt{agreed. see ->} \added{We demonstrate how to teach text-based agents to follow instructions by equipping RL agents with an internal structured representation in the form of Linear Temporal Logic (LTL) of the instructions found within the natural language.}. LTL is a formal modal logic with time-based modalities and binary predicates that dictate the events of the world (e.g. have-apple). LTL is able to expressively represent goals (or sequences of goals) and can -- through a mechanism called \textit{LTL progression} -- update goals that are yet to be satisfied while preserving the semantics of the original goal(s).
% \rephrase{LTL is an expressive formal language that combines temporal modalities such as eventually, until, and always with binary predicates that establish the truth or falsity of an event or property (e.g., have-coffee), composed via logical connectives to support specification of goal sequences, partial-order tasks, safety constraints, and much more. Our learning algorithm exploits a semantics-preserving rewriting operation, called LTL progression, that allows the agent to identify aspects of the original instructions that remain to be addressed in the context of an evolving experience.} 
%\remove{permits agents to learn the causal effects of their text-based actions through progression, which}
\revisit{We augment the GATA model using LTL to} allow it to condition on this structured representation over time and hypothesize that through progression, LTL  enables agents to \revisit{learn to follow instructions}. Our contributions are as follows:
\begin{itemize}
    % \item We in introduce a framework for teaching text-based RL agents how to follow instructions using LTL, built of \comment{LTL2Action}{Pop to a higher-level discussion of needing a symbolic representation of instructions and progression to inform the decision-making.} \cite{vaezipoor2021ltl2action}.
    \item We present our findings that show how current agents fail to follow instructions, leading to uninformed decision making in text-based games.
    \item We demonstrate the benefits of a formal representation of instructions (using LTL) for more informed decision-making in text-based games. We show how this approach greatly improves performance over state-of-the-art without increasing model complexity. \commentmt{Do we want to argue the "model complexity" as another benefit? If not remove this sentence maybe. }
    % \commenttk{Demonstrating that a formal representation of instructions improves performance doesn't mean that such a representation was \emph{needed}.\commentmt{Good point, changed to benefits}}
    \item We further show how the use of LTL progression is \added{a} critical mechanism that enables agents to realize their goals.
    % \item \added{We introduce a novel episodic exploration reward based on the set of environment objects that are relevant to the agent's goal?}
    % \item We demonstrate how this approach greatly improves performance over state-of-the-art. \commenttk{Maybe this should be part of the second point? Are the benefits referred to there different from greatly improved performance?}
\end{itemize}

==> sections/old_method.tex <==
% Scott: 
\section{Method}

In order to evaluate the impact of semantically encoding instructions for text-based games, 
we augment the GATA architecture for TextWorld~\citep{adhikari2020learning} with an LTL form of the instructions and a progression operator to track temporal progress through the instructions as the agent proceeds.  We will subsequently demonstrate that GATA can learn to leverage this progressed LTL augmented state to \emph{significantly} improve performance.
%we now describe our methodology to augment the aforementioned GATA architecture for TextWorld~\citep{adhikari2020learning} with an LTL-encoding of instructions and progress information.  

% PREVIOUS DISCUSSION, FOR REFERENCE
%build on the To date, the state-of-the-art (SOTA) model-free RL agent for TextWorld is the Graph Aided Transformer Agent (GATA) \citep{adhikari2020learning}. GATA uses a transformer variant of the popular LSTM-DQN \cite{narasimhan2015language} combined with a dynamic belief graph that is inferred and updated during planning. The aim is to use the dynamic belief graph to improve action selection by modelling the underlying game dynamics \citep{adhikari2020learning}. Formally, given the POMDP $<S, T, A, O, \Omega, R, \gamma>$, GATA attempts to learn some optimal policy $\pi^*(a | s, g)$ where $g$ is the belief graph of the agent.

\subsection{Model Architecture and Notation}
\label{sec:model_architecture}

% Under the hood, our DDQN agent uses
% \begin{itemize}
%     \item Transformer-based encoders \cite{vaswani2017attention} for all text-encoding, with normal positional encodings.
%     \item For word embeddings, we use the 300-dimensional fastText \cite{mikolov2017advances} word vectors trained on Common Crawl (600B Tokens). These are kept fixed during training.
%     \item and a simple 2-layer MLP with a ReLU non-linear activation function in between
%     \item We experiment with different encoding schemes
%     \begin{itemize}
%         \item Sharing the same text-encoder for observations, actions, and LTL
%         \item Independent text-encoders for observations, actions, and LTL
%     \end{itemize}
% \end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/model/flow.pdf}
    \caption{An example of single step during an episode of TextWorld. The game environment returns an observation $o_t$ and action candidate set $C_t$ in response to some action $a_{t-1}$. In turn, the agent's graph updater (GATA) updates its belief graph $g_t$ in response to both $o_t$ and $g_{t-1}$. Next, $g_t$ and $o_t$ update the LTL instructions.  $\varphi_t$ is generated from $o_t$ after the cookbook is examined and thereafter $\varphi_{t-1}$ is progressed to $\varphi_{t}$ at each time step.
    The policy network selects action $a_t$ from $C_t$ condition on $o_t$, $\varphi_t$, and $g_t$ and the cycle repeats.} 
    \label{fig:data_flow}
\end{figure}
We build a similar model to GATA's original architecture, augmented to include an LTL encoding of instructions. We dub this model \agentname. \autoref{fig:data_flow} visualizes an episode step interaction of LTL-GATA with TextWorld and \autoref{fig:model} visualizes the model itself. Additional details can be found in \autoref{sec:app_model}.

Before we describe details of the model, we introduce formal notation.  Formally, given the POMDP $<S, T, A, O, \Omega, R, \gamma>$, a set of finite propositional symbols $\mathcal{P}$, a labelling function $L : S \times A \rightarrow 2^{\mathcal{P}}$ that assigns truth values to the propositions in $\mathcal{P}$, $\sigma_j = L(s_j, a_j), ~j \in [1, \hdots, t]$, belief state $and LTL instructions $\varphi \in \Phi$, we aim to learn an optimal policy $\pi^*(a|s, g, \varphi)$.
%that follows these instructions. 
During an episode, the LTL representation $\varphi$ is generated and progressed using the observations and belief state. 
%We use a similar goal generator proposed in \cite{liu2022learning} to generate the instructions. 
%\commentmt{How do we want to frame this? First class citizen instructions?}. 
Finally, we make use of GATA's belief graph as our labelling function $L$.

With notation now defined, we proceed to describe individual components of  \autoref{fig:model} as well as the overall reinforcement learning approach.
%We defer more detailed discussions of the specific LTL encoding of instructions as well as reward structure and episode termination to Sections~\ref{sec:ltl_gen} and~\ref{sec:reward_episode_termination}, respectively.

%GATA does a very good job of accurately modelling the relations between objects in the world (i.e. identify truth assignments) and is well suited for progression of our instructions. We specifically use the GATA-GTP model, which generates a discrete belief graph composed of triplets that model object-relationship-object relations.
% \commenttk{I guess the $\varphi_{i,t}$ notation is meant to refer to result of progressing $\phi_i$ at the $t$-th time step?}
% \commenttk{Is $\Phi$ the set of \emph{all} LTL formulas? The reward in Option 1 below seems to suggest we want to make them all true, so maybe it's just the formulas we want to satisfy in one episode. But then why is the policy conditioned on a particular formula?}  \commentmt{A game can have multiple sets of formulaes: e.g. [(next cookbook\_is\_examined), (and eventually onion\_in\_player meal\_is\_consumed)], so $\Phi$ is that list/set. Because once we progress the first one to completion, the second one is used and progressed.}

\textbf{Graph Updater:} This component represents the original GATA model. 
We specifically 
use the GATA-GTP model~\citep{adhikari2020learning}, which generates real-valued beliefs over triplets  $(\mathit{object},\mathit{relationship},\mathit{object})$ of the knowledge state of the world, e.g., $(\textit{red potato},\mathit{is},\mathit{chopped})$.
The graph updater for these triplets is specifically composed of two components: (a) the actual graph updater that generates the belief state updates. These generate $g_t$ from observation $o_t$ and the graph $g_{t-1}$; and (b) the graph encoder. The graph encoder encodes the current graph as $\texttt{GE}(g_t) = g'_t \in \mathbb{R}^D$ for $D$ triplets. The graph encoder is a relational graph convolutional network (R-GCN) \citep{schlichtkrull2018modeling} using basis regularization \citep{schlichtkrull2018modeling} and highway connections \citep{srivastava2015highway} between layers for improved convergence. We refer the readers to \cite{adhikari2020learning} for more details.

% \commenttk{\cite{liu2022learning} didn't use LTL, did they? I think we need a lot more detail on how the instructions are generated.}\commentmt{No, they used plain english forms of the goal, but used a similar rule-based method. In terms of more information, yeah it depends how we think it best to frame this. Liu et all just metnioned they had a goal extractor and move description to the appendix. Unless we want to be upfront and talk about how this is "first class citizen" advice/instructions or something. I've moved describption of the instruction generation to sec 3.2}
\textbf{LTL Updater:}  
The LTL updater generates and progresses LTL instructions $\varphi_t$ .  In brief, LTL instructions defining the need to arrive at the kitchen and examine the cookbook are generated from $o_0$. The subsequent instruction defining the recipe is generated from game observation $o_t$ (to be described in \autoref{sec:ltl_gen}) when the action $\textit{examine cookbook}$ is executed at time $t$. For truth assignment (i.e. the labelling function $L$) needed to progress the LTL, we leverage GATA's highly accurate belief state from the graph updater.
%directly use the a discrete graph GATA model (GATA-GTP). 
We use use the Spot \citep{spotsoftware} engine to perform the progression.

%GATA-GTP accurately tracks when recipe steps have been achieved and hence we use it directly for progression of $\varphi$.

\textbf{Text Encoders:} For encoding the action choices $C_t$, observations $o_t$, as well as encoding the LTL instructions $\varphi_t$, we use a simplified version of the Transformer architecture presented in \cite{vaswani2017attention}. This is the same architecture used in \citep{adhikari2020learning}. For LTL instructions, we encode them directly as a string. For example, the LTL formula
\begin{align*}
    \varphi: \ltleventuallyTXT p_1 \wedge \ltleventuallyTXT p_2
\end{align*}
where $p_1=\ltlpredicate{pepper-in-player}$ and $p_2=\ltlpredicate{pepper-is-cut}$, has the string representation 
\begin{align*}
    \text{str}(\varphi): ``\text{eventually player\_has\_pepper and eventually pepper\_is\_cut}``
\end{align*}
Importantly, we format each predicate as a single token. The word embedding of each token is the average of the word embeddings for each underscore-separated token in the predicate. We show in \autoref{sec:app_exp_pred} that our method is robust to predicate format.
% \commentmt{tmp example, needs work. make sure formalism is consistent with prior examples}.
% \commenttk{Why does the text string have one ``eventually'' when there were two in the formula?}
% \commentmt{typo - fixed} 

For some vector $v \in \mathbb{R}^{d}$ the transformer (text encoder) outputs a single vector $\texttt{Tr}(v) = v' \in \mathbb{R}^D$ of dimension $D$, which is the same dimension as the graph encoder. \commenttk{Are $d$ and $D$ different?s}

\textbf{Action Selector:}  The action selector is a 2-layer multi-layer perceptron (MLP).The encoded state vectors $\texttt{Tr}(o_t) = o_t' \in \mathbb{R}^D$, $\texttt{Tr}(\varphi_t) = \varphi_t' \in \mathbb{R}^D$, and $\texttt{GE}(g_t) = g_t'\in \mathbb{R}^D$ are concatenated to form the final state representation $s_t = [o_t';\varphi_t';g_t'] \in \mathbb{R}^{3D}$. This vector representation is then concatenated with the encoded action choices $C_t'\in \mathbb{R}^{n_c\times D}$ where $n_c$ is the number of action choices. This concatenation occurs by repeating the state's vector representation $n_c$ times and then concatenating. This final concatenated representation is fed to the MLP which returns a vector $q_c \in \mathbb{R}^{n_c}$, which represents the q-values for each action choice. Finally, we note that in contrast to GATA's work, we contenate features rather than use the bi-directional attention-based aggregator \cite{adhikari2020learning}. We found experimentally that contenation worked just as well and simplified the model's complexity.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figures/model/policy_model.pdf}
    \caption{\agentname's policy model. The model chooses action $a_t \in C_t$ conditioned on the state $s_t = [o_t';\varphi_t';g_t']$. The action selector chooses $a_t$ based on the predicted Q-values.}
    \label{fig:model}
\end{figure*}
% Consider a single example (or batch size $=1$). For some time step $t$, the TextWorld returns an text-based observation $o_t$, which has associated text-based LTL instruction $\varphi_{i,t}$, and set of admissible actions $\admissibleActions_t$, $|\admissibleActions_t| = Z$. A forward pass through our agent's model then looks as follows:
% \begin{align*}
%     h_{o_t} &= \texttt{Transformer}(o_t);~\in \mathbb{R}^{L_{o_t}\times W}\\
%     h_{\varphi_{i,t}} &= \texttt{Transformer}(\varphi_{i,t});~\in \mathbb{R}^{L_{\varphi_{i,t}}\times W}\\
%     h_{\admissibleActions_t} &= \texttt{Transformer}(\admissibleActions_t);~\in \mathbb{R}^{Z\times L_{\admissibleActions_t}\times W}\\
%     \hat{h}_{o_t} &= \texttt{stack}[h_{o_t} \times Z]~\in \mathbb{R}^{Z\times L_{\admissibleActions_t}\times W}\\
%     \hat{h}_{\varphi_{i,t}} &= \texttt{stack}[h_{\varphi_{i,t}} \times Z]~\in \mathbb{R}^{Z\times L_{\admissibleActions_t}\times W}\\
%     a_{i,t} &= \argmax~\texttt{SOFTMAX}\left(\texttt{MLP}(\texttt{concatenate}[h_{\admissibleActions_t}, \hat{h}_{o_t}, \hat{h}_{\varphi_{i,t}}])\right)
% \end{align*}
% where $L_{o_t}$ is sequence length of the observations, $L_{\varphi_{i,t}}$ is the sequence length of the LTL instruction, $L_{\admissibleActions_t}$ is the max sequence length of the actions in the set of admissible actions, $Z$ is the number of admissible actions, and $W$ is the output embedding size of our Transformer encoder. 
\textbf{Training.} For training, we implement Double DQN (DDQN) \cite{van2016deep} with reward function and termination criteria as discussed in \autoref{sec:reward_episode_termination}. We use a prioritized experience replay buffer \cite{schaul2015prioritized} that collects transitions from randomly sampled games. We refer the reader to \autoref{sec:app_training} for further training details.

%\subsection{Playing Text-Based Games with LTL}
%\label{sec:tbg_and_ltl}
% Within an episode, instructions can get revealed as the agent acts and interacts in the environment. In the context of the Cooking domain, the agent is first instructed to go and examine the cookbook which then elicits a recipe that it needs to follow. This ultimately defines the goals the agents needs to accomplish to succeed in the game.

%Our method is simple: generate and progress LTL instructions and allow the agent to condition on them as part of its state representation. Formally, given the POMDP $<S, T, A, O, \Omega, R, \gamma>$, a set of finite propositional symbols $\mathcal{P}$, a labelling function $L : S \times A \rightarrow 2^{\mathcal{P}}$ that assigns truth values to the propositions in $\mathcal{P}$, $\sigma_j = L(s_j, a_j), ~j \in [1, \hdots, t]$, and LTL instructions $\varphi \in \Phi$, our agent's goal becomes to learn some optimal policy $\pi^*(a|s, g, \varphi)$ that follows these instructions. During an episode, $\varphi$ is generated and progressed using the observations and belief state. We use a similar goal generator proposed in \cite{liu2022learning} to generate the instructions. \commentmt{How do we want to frame this? First class citizen instructions?}. Finally, we make use of GATA's belief graph as our labelling function $L$. GATA does a very good job of accurately modelling the relations between objects in the world (i.e. identify truth assignments) and is well suited for progression of our instructions. We specifically use the GATA-GTP model, which generates a discrete belief graph composed of triplets that model object-relationship-object relations.
% \commenttk{I guess the $\varphi_{i,t}$ notation is meant to refer to result of progressing $\phi_i$ at the $t$-th time step?}
% \commenttk{Is $\Phi$ the set of \emph{all} LTL formulas? The reward in Option 1 below seems to suggest we want to make them all true, so maybe it's just the formulas we want to satisfy in one episode. But then why is the policy conditioned on a particular formula?}  \commentmt{A game can have multiple sets of formulaes: e.g. [(next cookbook\_is\_examined), (and eventually onion\_in\_player meal\_is\_consumed)], so $\Phi$ is that list/set. Because once we progress the first one to completion, the second one is used and progressed.}

\subsection{Generating and Formatting the Instructions for TextWorld}
\label{sec:ltl_gen}
We use two types of instructions for the Cooking domain. The first instruction identifies the need to examine the cookbook: This instruction is complete and is defined as
\begin{align*}
    \varphi: \ltlnextTXT \ltlpredicate{cookbook-is-examined}.
\end{align*}
This instruction simply states that the predicate $\ltlpredicate{cookbook-is-examined}$ should be true in the next step of the game. The second instruction is the actual recipe that gets elicited from the cookbook. We format this instruction to be (a) order-invariant and (b) incomplete. Order-invariance allows the agent to complete the instructions in any order, but is still constrained by any ordering that the TextWorld engine may enforce, and \comment{incompleteness is a relaxation on when an instruction should be completed}{TK: What does this mean?}. Assuming the recipe requires that predicates $p_1, p_2, \hdots p_n$ be true, the cookbook instructions are modelled as
\begin{align*}
    \varphi: (\ltleventuallyTXT p_1) \wedge (\ltleventuallyTXT p_2) \wedge \hdots (\ltleventuallyTXT p_n).
\end{align*}
% \commenttk{I'm not sure the scope of the operators is clear. Is the scope of each $\ltleventuallyTXT$ just the next $p_i$, or everything to the right? I guess from the informal description it's the former.} \commentmt{yes, scope is $p_i$ directly next to operator. The instructions, once finally processed by spot, actually get converted to normalized Polish notation (I think that's what it's called). Perhaps I should desccribe and use that notation, but it's not as "clear"}.
For example, in the Cooking Domain, this instruction might be
\begin{align*}
    \varphi: (\ltleventuallyTXT \ltlpredicate{\scriptsize{apple-in-player}}) \wedge 
             (\ltleventuallyTXT \ltlpredicate{\scriptsize{meal-in-player}}) \wedge 
             (\ltleventuallyTXT \ltlpredicate{\scriptsize{meal-is-consumed}}).
\end{align*}

% \commentpv{After reading this section it's still not clear to me how the instructions of the second type are generated from the text instructions. We ideally want to emphasize that this is done mechanically.}
% \commentmt{I've been 'avoiding' that, but perhaps you're right and just be upfront about it is best. The ICLR work moved the actually description to the supp material but perhaps that's not the best course of action in our case. See below for a (wordy) intial description.}

In this work, we generate these instructions mechanically, exactly like the goal generation method used by \cite{liu2022learning}. TextWorld's observations are easily parsed to extract the goal information already contained within them, which we then formalize and keep track of using LTL. We specifically only ever generate three instructions: (1) the need to check the cookbook, which is generated from the initial game observation: (2) the recipe instruction, which is generated from the observation following an agent examining the cookbook: and (3) a finding kitchen instruction, which is also generated from the initial game observation and only applies on certain game level. We provide examples of these observations and more details in \autoref{sec:app_ltl_generation}. Note that these observations are only used to generate the \textit{initial} instruction, and subsequently LTL progression is used with the GATA belief state to update and progress those instructions.

\subsection{Rewards and Episode Termination}
\label{sec:reward_episode_termination}
% For the DDQN algorithm employed in this work, rewards are step-based. Below, we formulate the reward functions as the total accumulated reward up to the given time step $t$, but in practice, the agent is only reward on a step-by-step basis, hence, the reward $r_t$ given to the agent at any time step $t$ is the difference in accumulated rewards between two steps, or 

% Recall our reward function returns the total accumulated reward, however in practice, DDQN uses a step-based reward $r_t$ where $t$ is the current step in the game episode. We define this step-based reward as
% \begin{align*}
%     r_t = R_{\Phi}(s_1, a_1, \hdots, s_t, a_t) - R_{\Phi}(s_1, a_1, \hdots, s_{t-1}, a_{t-1})
% \end{align*}
% where $R(s_1, a_1, \hdots, s_t, a_t)$ is the total accumulated reward at step $t$. We define $R_{\Phi}$ as follows: 
% \commenttk{I'm not sure why we couldn't just have $r_t=R_{\Phi}(s_1,a_1,\hdots,s_t,a_t)$. Is this to make the bonus rewards in Option 1 below interpretable as potential-based reward shaping or something like that?}
% \commentmt{In this case I'm using R() to define the total accumulated reward. I just find it easier to develop the formalism around this way. I could be wrong.}

In addition to augmenting the agent's state representation, we can also reward our agent for completing instructions, which we model as $R_{\Phi}(s,a,\varphi)$. For some labelling function $L : S \times A \rightarrow 2^{\mathcal{P}}$ that assigns truth values to the propositions in $\mathcal{P}$, and $\sigma_j = L(s_j, a_j), ~j \in [1, \hdots, t]$
% \begin{align*}
%     R_{\Phi}(s_1, &a_1, \hdots, s_t, a_t)  =R(s_1, &a_1, \hdots, s_t, a_t) + 
%     \begin{cases}
%     \sum\limits^n_{i=0} \mathbb{I} [\sigma_1\hdots\sigma_t \models \varphi_i]\\
%     -1 ~~ \text{if}~ \sigma_1\hdots\sigma_t \models \neg\varphi_0 \vee \hdots  \vee  \neg\varphi_n\\
%     \end{cases}
% \end{align*}
\begin{align*}
    R_{\Phi}(s, a, \varphi)  =R(s, a) + 
    \begin{cases}
    1 ~~ \text{if}~ \mprog(L(s,a), \varphi) = \true\\
    -1 ~~ \text{if}~ \mprog(L(s,a), \varphi) = \false\\
    0 ~~ \text{otherwise}
    \end{cases}
\end{align*}
In other words, a bonus reward is given for every LTL instruction the agent satisfies a penalty is given if the agent fails to complete an instruction. We perform an ablative study on the effect of this reward in \autoref{sec:exp_reward_term}. We henceforth refer to this modified reward function as the \textit{LTL reward}.

Further, because we wish to \textit{satisfy} instructions, we can also use the instructions to modify episode termination. That is, if our LTL instruction is said to be violated, we have arrived in a terminal state, even if the TextWorld engine does not recognize this as a terminal state. We similarly perform an ablative study on the effect this modified episode termination in \autoref{sec:exp_reward_term}. We henceforth refer to this modified episode termination as \textit{LTL-based termination}.
% \commenttk{Does the LTL formula actually have an influence on the termination conditions, or is it just that we choose it to match what the termination conditions already were? If it does influence termination, that goes beyond just determining the reward.}

% \commentmt{Yes, LTL \textit{can} have an influence on termination (e.g. next examine\_cookbook, if you don't episode terminates.). Should perform ablation on the effect of ltl-termination vs. not.}

% \textbf{Option 2: No LTL reward.} Idea: this is simply the original game reward with no LTL-based bonus of any kind. We experiment with this reward scheme to also demonstrate that there are benefits to rewarding the agent for progressing through its LTL instructions, however including the LTL formula as part of the state is more important. We demonstrate that by showing that not rewarding for LTL progression still achieves good performance levels.
% \begin{align*}
%     R_{\Phi}(s_1, 
%     a_1, \hdots, s_t, a_t)  = R
% \end{align*}
% \commenttk{I guess $R$ is the original reward function $R(s_t,a_t)$? But then the step-based reward as described above is $r_t=R(s_t,a_t)-R(s_{t-1},a_{t-1})$ which wouldn't be equal to $R(s_t,a_t)$ in general.}
% \textbf{Option 2: Reward LTL only}
% Idea: only the sparse LTL satisfaction (or violation) rewards are given, with no additional bonus from the game rewards. 
% \begin{align*}
%     R_{\Phi}(s_1, &a_1, \hdots, s_t, a_t)  = \\&
%     \begin{cases}
%     \sum\limits^n_{i=0} \mathbb{I} [\sigma_1\hdots\sigma_t \models \varphi_i]\\
%     -1~~ \text{if}~ \sigma_1\hdots\sigma_t \models \neg\varphi_0 \hdots  \vee \neg\varphi_n\\
%     \end{cases}
% \end{align*}

% \textbf{Option 3: Reward Bonus but Stop on Violation}
% \begin{align*}d
%     R_{\Phi}(s_1, &a_1, \hdots, s_t, a_t)  = \\&
%     \begin{cases}
%     R + \sum\limits^n_{i=0} \mathbb{I}[\sigma_1\hdots\sigma_t \models \varphi_i]\\
%     -1~~ \text{if}~ \sigma_1\hdots\sigma_t \models \neg\varphi_0 \vee \hdots  \vee \neg\varphi_n\\
%     \end{cases}
% \end{align*}

% \textbf{Option 1: Reward LTL as bonus for each progression}
% Idea: use the ltl rewards as bonuses in the step rewards. Here though, an LTL reward (of 1) is given for each succesful progression of the each subgoal formula. This is similar to Option 1, except that each progression is rewarded rather than the entire subgoal formula needing to be satisfied before getting any bonus.
% \begin{align*}
%     R_{\Phi}(s_1, &a_1, \hdots, s_t, a_t)  = \\&R + 
%     \begin{cases}
%     \sum\limits^n_{i=0} ??\\
%     -1 ~~ \text{if}~ \sigma_1\hdots\sigma_t \models \neg\varphi_0 \vee \hdots  \vee  \neg\varphi_n\\
%     \end{cases}
% \end{align*}

% \textbf{Option 5: Reward only if all formulae satisfied}
% Idea: because there may be multiple LTL formula that define different subgoals, this is a sparser version of option 1 where you only get a bonus of $1$ if all these formula are satisfied over the course of the episode, rather than a bonus for each subgoal-formula.
% \begin{align*}
%     R_{\Phi}(s_1, &a_1, \hdots, s_t, a_t)  = \\&R + 
%     \begin{cases}
%     1 ~~ \text{if}~ \sigma_1\hdots\sigma_t \models \varphi_0 \wedge \hdots \wedge \varphi_n\\
%     -1 ~~ \text{if}~ \sigma_1\hdots\sigma_t \models \neg\varphi_0 \vee \hdots  \vee  \neg\varphi_n\\
%     0 ~~ \text{otherwise}
%     \end{cases}
% \end{align*}

